Synthesis and verification of robust-adaptive safe controllers

Safe control with guarantees generally requires the system model to be known. It is far more challenging to handle systems with uncertain parameters. In this paper, we propose a generic algorithm that can synthesize and verify safe controllers for systems with constant, unknown parameters. In particular, we use robust-adaptive control barrier functions (raCBFs) to achieve safety. We develop new theories and techniques using sum-of-squares that enable us to pose synthesis and verification as a series of convex optimization problems. In our experiments, we show that our algorithms are general and scalable, applying them to three different polynomial systems of up to moderate size (7D). Our raCBFs are currently the most effective way to guarantee safety for uncertain systems, achieving 100% safety and up to 55% performance improvement over a robust baseline.

==> old_files/method_syn.tex <==
\subsection{raCBF synthesis}\label{sec:methodology:synthesis}

In this section, we provide an algorithm for synthesizing an raCBF given the partially defined system (Eq.~\ref{eqn:sys_dynamics}), the safety definition (Eq.~\ref{eqn:sys_safety_def}), and a feasible initialization for the raCBF. We would like to find $\phi(x, \hat{\theta})$ satisfying Theorem~\ref{thm:valid_raCBF}, where $\phi$ is now a polynomial of fixed degree over $x, \theta$ with variable coefficients. However, with $\phi$ containing optimization variables, Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}),~(\ref{eqn:subset_constraint}) are no longer convex, but bilinear. This requires us to apply bilinear alternation on these constraints, which form the basis of our Alg.~\ref{alg:raCBF}. 

While bilinear alternation alone would yield a {\it valid} raCBF, we'd also like the raCBF to capture a large invariant set. A larger invariant set means the system is less restricted, providing the nominal controller more flexibility. Thus, our optimization needs to also maximize the size of the invariant set $\mathcal{I}^{r}_{\hat{\theta}}$. To do this, we follow~\cite{dai2022convex}. To increase its size, we perform several steps in each iteration. First, we find the largest ellipsoid $\mathcal{E}_r \defeq \{x \mid x^{\top}P x \leq r\}$ contained within $\mathcal{I}^{r}_{\hat{\theta}}$ (solve SOSP~\ref{eqn:phase1} for the maximum ellipsoid radius $r$). Then, we optimize the raCBF so that the margin between 
$\mathcal{E}_r$ and $\mathcal{I}^{r}_{\hat{\theta}}$ is as large as possible (SOSP~\ref{eqn:phase2}). This effectively increases the size of $\mathcal{I}^{r}_{\hat{\theta}}$ over the iterations. We also add an ``anchor constraint'', which limits the maximum value of the raCBF. This helps us avoid a trivially optimal raCBF with large values but a small invariant set. We also do bilinear alternation: SOSP~\ref{eqn:phase2} optimizes the multipliers $s_i(x, \theta), r_i(x, \theta)$ and then SOSP~\ref{eqn:phase3} optimizes the raCBF $\phi(x,\hat{\theta})$, and back and forth. 

Another challenge posed by synthesis is the requirement for a feasible initialization. That is, we need to supply a raCBF already satisfying Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}),~(\ref{eqn:subset_constraint}) when using bilinear alternation. Generally, this initialization is something that can be computed straightforwardly, but has a trivially small invariant set. Then, the idea is for synthesis to enlarge the invariant set, while maintaining validity, until the raCBF is usable. We can easily provide such an initialization if the robust range $\Theta$ is small. In that case, we can use the control Lyapunov function (CLF) corresponding to a linear quadratic regulator (LQR) which stabilizes to an equilibrium point in $\mathcal{X}_{\text{safe}}$. This initialization will intrinsically have some robustness to perturbation~\cite{chen2015robustness}. However, in the general case, the robust range $\Theta$ will have moderate size. 

To handle this, we consider a small robust range at initialization, so that we may use our LQR-based CLF initialization. Then, we maximize this robust range over the iterations (SOSP~\ref{eqn:phase3}). In our experiments, the ultimate robust range produced by our algorithm is always equal to the desired range, which is set using commonly known ranges for the physical parameters. However, we have found, for example, that the algorithm is unable to increase the robust range to double the desired size. This is not a significant issue though, since robust control is generally not recommended when the desired range is large~\cite{lavretsky2012robustAdaptive}.

{\small
\begin{subequations}

\begin{align}
    &\textbf{Phase 1 (P1)} \label{eqn:phase1} \\
    & \max_{r\in\mathbb{R}, s_0 \in \Sigma} r \nonumber \\
    & s.t.\;\; x^{\top} P x - r - s_0 \phi \in \Sigma \nonumber \\ \notag \\ 
    & \textbf{Phase 2 (P2)} \label{eqn:phase2} \\
    & \min_{s_i, r_i \in \Sigma, t \in \mathbb{R}} t \nonumber\\
    % & \text{s.t. for}\; x \in \mathcal{X}, \theta \in \Theta \nonumber \\ 
    &c + d \bar{u} - s_1 d - s_2 (\phi - \beta^{-}) \in \Sigma \nonumber \\ 
    &c + d \ubar{u} + s_3 d - s_4 (\phi - \beta^{-}) \in \Sigma \tag*{Control filter feas. constraints} \\
    &\phi - r_i b_i \in \Sigma \;\;,\; \forall i=1,\ldots,t \tag*{Subset constraints}\\
    &t - \phi - s_5 (r - x^{\top} P x) \in \Sigma \tag*{Ellipsoid constraint}\\
    &1 - \phi(0, \theta) \in \Sigma \tag*{Anchor constraint} \\ \notag \\
    & \textbf{Phase 3 (P3)}\label{eqn:phase3} \\
    & \min_{\phi, t, \theta_l, \theta_u}ƒ t + \theta_l - \theta_u \nonumber \\
    % & \text{s.t. for}\; x \in \mathcal{X}, \theta \in \Theta \nonumber \\ 
    &c(x, \theta) + d(x, \theta) \bar{u} - s_1 d(x, \theta) - s_2 (\phi - \beta^{-}) \in \Sigma \nonumber \\ 
    &c(x, \theta) + d(x, \theta) \ubar{u} + s_3 d(x, \theta) - s_4 (\phi - \beta^{-}) \in \Sigma \tag*{Control filter feas. constraints} \\
    &\phi - r_i b_i \in \Sigma \;\;,\; \forall i=1,\ldots,t \tag*{Subset constraints}\\
    &t - \phi - s_5 (r - x^{\top} P x) \in \Sigma \tag*{Ellipsoid constraint}\\
    &1 - \phi(0,\theta) \in \Sigma \tag*{Anchor constraint}
\end{align}
\end{subequations}
}



==> old_files/method_verif.tex <==
\subsection{raCBF verification}\label{sec:methodology:verification}
% Subsection A: raCBF verification
In this section, we derive an SOSP that allows us to verify if a given raCBF satisfies Theorem~\ref{thm:valid_raCBF}. Our goal is to convert Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}),~(\ref{eqn:subset_constraint}) into the form of Eq.~(\ref{eqn:sosp_constraints}).

Looking first at Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}), we see that it requires us to show that for all $x \in \mathcal{X}, \theta \in \Theta$, there exists some $u \in \mathcal{U}$ satisfying the constraint. The ``exists'' quantifier complicates the conversion, as theorems like P-satz and S-procedure can only support “for all” quantifiers. However, it turns out that for any $x$, we can identify which $u \in \mathcal{U}$ achieves the supremum in Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}) - call it $u^{*}(x)$. Therefore, we only need to check whether Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}) is satisfied for $u^{*}(x)$ for all $x$. 

We derive $u^{*}(x)$ by regarding Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}) as a constrained optimization over the input $u$. In fact, it is a special kind of optimization problem with an affine objective and a compact, convex constraint set. Hence, the maximizer always occurs at a vertex of the constraint set~\cite{dantzig2002linear}, $\defeq v^j$ where  $v_i^j \in \{\ubar{u}_i, \bar{u}_i\}$. For each $x$, we can further identify which vertex is the maximizer. First, we write Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}) more clearly in control-affine form. Let {\small $\c(x, \hat{\theta}) \defeq \nabla_{x} \phi(x, \hat{\theta}) (f - \Delta \hat{\theta} ) + \alpha ( \phi(x, \hat{\theta}) - \tfrac{1}{2\gamma}\tilde{\theta}^{\top}\tilde{\theta} )$} and {\small $d(x, \hat{\theta}) \defeq \nabla_{x} \phi(x, \hat{\theta}) g(x)$}, so that Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}) can be rewritten as {\small $\sup_{u \in \mathcal{U}} c(x, \hat{\theta}) + d(x, \hat{\theta}) u$}. For $i = 1, \ldots, m$, if $d(x, \theta)_i \geq 0$, i.e., the $i$\textsuperscript{th} entry of vector $d(x, \theta)$ is nonnegative, then $u^{*}_{i}(x) = \bar{u}_i$ and vice versa. There are then $2^m$ groups of $x$ with distinct sign patterns on $d(x, \theta)$ that have distinct maximizers $u^{*}(x)$. Hence, we can write $2^m$ constraints for all the groups of $x$.

We give an example for $m = 1$, although the general case is an immediate extension. We have two constraints:
\begin{align}
    & \forall x \in \mathcal{X}, \theta \in \Theta, \;\;\text{s.t.}\;\; \phi(x, \theta) \geq \beta^{-}: \nonumber \\
    & d(x, \theta) \geq 0 \implies c(x, \theta) + d(x, \theta) \bar{u} \geq 0 \\
    & d(x, \theta) \leq 0 \implies c(x, \theta) + d(x, \theta) \ubar{u} \geq 0
\end{align}

Applying the S-procedure gives us the following SOSP constraints: 
\begin{align}
    c + d \bar{u} - s_1 d-s_2(\phi - \beta^{-}) \in \Sigma, \;\; s_1, s_2 \in \Sigma \label{eqn:sosp_constraint_u1} \\ 
    c + d \ubar{u} + s_3 d-s_4(\phi - \beta^{-}) \in \Sigma, \;\; s_3, s_4 \in \Sigma \label{eqn:sosp_constraint_u2} 
\end{align}

Likewise, we can also apply the S-procedure to \eqref{eqn:subset_constraint} to yield:
\begin{align}
    \phi(x, \theta) - r_i b_i \in \Sigma ,\;\; \forall i=1,\ldots,t \;,\; r_i \in \Sigma \label{eqn:sosp_constraint_subset}
\end{align}


% \sum_{i = 1}^{p} s_i^{-} (\theta_i - \ubar{\theta}_i) 

\begin{Theorem}[raCBF verification]
For the case where $m=1$\footnote{The case for general $m$ is an immediate extension, but omitted for notational brevity.}, a polynomial $\phi(x, \hat{\theta})$ is a valid raCBF, providing set invariance and finite-time convergence in $\{x | \phi \geq \beta^{-}\}$, if there exists $s_{1:4}, r_i$ such that the convex constraints in Eq.~(\ref{eqn:ctrl_fltr_feas_constraint}) and~(\ref{eqn:subset_constraint}) are satisfied. This can be determined by seeing if the SOSP consisting of constraints~(\ref{eqn:sosp_constraint_u1}),~(\ref{eqn:sosp_constraint_u2}),~(\ref{eqn:sosp_constraint_subset}) is feasible.         
\end{Theorem}
% Theorem 2 (?): For the case where m = 1:






==> old_files/old_abstracts.tex <==
To design a guaranteed safe controller, we are typically required to know the system model. However, a known model is an unrealistic assumption. In this paper, we consider the more challenging scenario of designing safe control for uncertain systems. We propose a generic algorithm that can verify and synthesize safe controllers for any polynomial systems with constant, unknown parameters. In particular, we use robust-adaptive control barrier functions (raCBFs) to achieve safety. Also, we use sum-of-squares programming to pose verification and synthesis as a series of convex optimization problems. 

Ultimately, we produce raCBFs that are less conservative compared to other approaches, enabling better performance at other control objectives besides safety (stabilizing, tracking). Our algorithm is also far more scalable, allowing us to handle systems of moderate dimension ($\leq$ 7D) compared to 2D as before. We illustrate on three systems: toy 2D with an unknown parameter and cartpole and quadrotor with unknown friction coefficients. We confirm via simulation that the raCBFs keep the systems 100\% safe, despite model uncertainty. 


% Safe control with guarantees generally requires the system model to be known. It is far more challenging to handle systems with uncertain parameters. In this paper, we propose the first generic algorithm that can verify and synthesize safe controllers for any polynomial systems with constant, unknown parameters. In particular, we utilize robust-adaptive control barrier functions (raCBFs) to achieve safety. We use sum-of-squares programming to pose verification and synthesis as a series of convex optimization problems. We illustrate our algorithm by synthesizing safe controllers for three systems: a toy 2D system with an unknown parameter, and a cartpole and quadrotor with unknown friction coefficients. We confirm via simulation that the raCBFs indeed keep the systems safe, despite model uncertainty. 

% TODO \\
% Note on crafting abstracts: Use it to clarify the vague terms in the title \\
% Uncertain systems $\rightarrow$ specifically, systems with parametric uncertainty (i.e. a fixed/time-invariant unknown parameter) \\
% Design/synthesize $\rightarrow$ specifically, use sum-of-squares programming to produce a CBF (why not have SOSP in the title itself?) \\
% This scheme also comes with an estimator for the uncertain parameter which Lopez had designed. (uCBF)


% This works proposes a method for synthesizing control barrier functions (CBF) for adaptive safe control of dynamical systems with parametric model uncertainties, i.e., fixed or time-invariant unknown parameters. This synthesis method generates adaptive controllers that guarantee safety under the actual dynamics via designing both the controller and the estimator \cite{lopez2023unmatched}. Our approach also accounts for the physical actuation limits to ensure that a safe control input exists even under uncertain systems. We utilize sum-of-squares programming (SOSP) to synthesize the CBF. We demonstrate our algorithm on three simulated systems - 2D toy polynomial system with unknown parameter, adaptive cruise control problem with unknown friction coefficients, and Acrobot system with unknown viscous friction terms.

==> old_files/old_conclusion.tex <==
In this paper, we proposed the first generic optimization algorithm for synthesizing safe controllers for systems with constant, unknown parameters. We showed that the constraints characterizing a valid raCBF can be written as an SOS program, and that we can write a multi-phase algorithm to find an raCBF with a large invariant set and robust range. We also showed that this algorithm is effective for a range of scenarios: systems with up to moderate dimension, multiple unknown parameters, multiple barrier functions, different relative degrees. 
Our simulations of the feedback control loop confirmed that the synthesized raCBFs do indeed keep the uncertain systems safe. In the future, we are interested in extending synthesis to systems with time-varying unknown parameters. 


==> old_files/old_intro.tex <==
% TODO: go back through and insert citations everywhere 
Safety is required for many systems whose dynamical models cannot be exactly known. For example, we would like to prevent collision for autonomous vehicles~\cite{funke2016collision}, drones~\cite{alvarez2015collision}, and manipulators~\cite{seraji1999real}, and all of these systems may have unknown friction or damping effects. These unknown effects pose a challenge for model-based safe control methods, like control barrier functions~\cite{ames2019control, wei2019safe}, which typically require perfect knowledge of the model. Our work addresses this problem. We provide an algorithm to synthesize robust adaptive CBFs (raCBFs), which ensure safety for systems with unknown parameters. This algorithm has the benefit of being generic, meaning it can synthesize raCBFs for all polynomial systems of moderate dimension ($\leq 7$D).

% Assumption paragraph
In our work, we consider systems that are polynomial and affine in the unknown parameters $\theta$ and also in the control input $u$, and with constant unknown parameters of the form: 
\begin{equation}
    \dot{x} = f(x) - \Delta(x) \theta + g(x) u .
\end{equation}
% <Insert system eqn>
Many robotic systems are actually of this form, so these are not restrictive assumptions. Namely, many models for manipulators, drones, and vehicles are either polynomial or can easily be transformed to polynomial form. Often, the most significant unknown parameters in these systems are frictional coefficients, which appear in an affine way. % and are constant.  

The technique we use is “sum-of-squares programming” (SOSP)~\cite{papachristodoulou2005tutorial,jarvis2003some}, which allows us to pose the search for a valid raCBF, given a partially-known system and a safety requirement, as a constrained optimization problem. This optimization problem can be broken down into a series of convex optimization problems, which can each be solved with an off-the-shelf semidefinite program (SDP) solver.  

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{final_figures/systems_side_by_side.jpg}
    \caption{Systems with uncertain parameters: cartpole (left) and 2D quadrotor (right). For cartpole, $m_c$ is the mass of cart, $m_p$ is the mass of pole, $l$ is the length of pole, $\psi$ is the pole angle, $x$ is the horizontal distance of the cart from the origin, and $u$ is the horizontal input force on the cart. For quadrotor, $x,y$ are the horizontal and vertical location of the quadrotor, $\psi$ is the angle of the body with respect to the positive $x$-axis, $r$ is the distance between the center of the quadrotor base and the propellor base, and $u_1,u_2$ are the two thrust input forces from the propellers. Cartpole has the joint's friction coefficient as the unknown parameter and quadrotor has the drag coefficients in the $x,y$ directions as the unknown parameters.}
    % \caption{Cartpole system with counter-clockwise rotation of the pole. $\psi$ is the angle between cart's center of mass and the pole. Zero-configuration is when the pole is pointing downwards with no movement such that $\psi=0,\dot\psi=0$. The joint connecting the pole and the cart is at the cart's center of mass.}
    \label{fig:systems_side_by_side}
\end{figure}

In control theory, uncertain systems are usually handled with adaptive, robust, or robust-adaptive control~\cite{lavretsky2012robustAdaptive}. In adaptive control, the controller depends on estimates of the unknown system. Typically, the system will be estimated online and the controller {\it adapts} with each new estimate. In robust control, the controller only depends on disturbance bounds that are known a-priori, which typically means the controller can be synthesized entirely offline. 

The robust and adaptive paradigms have different strengths and weaknesses. While robust control is known to compensate for uncertainties quickly, adaptive control compensates in a less conservative way, allowing the system more freedom~\cite{lavretsky2012robustAdaptive}. Robust-adaptive control combines the merits of both paradigms, compensating efficiently for uncertainty while avoiding conservatism. In general, robust-adaptive controllers can combine robust and adaptive elements in many different ways. Our scheme, in particular, uses a CBF that depends on the estimated system parameters and is robust to the largest possible estimation error. 

% A robust-adaptive control strategy combines the benefits of both: it is efficient while not being conservative, even when the bounds on unknown parameters are larger. Our raCBF is adaptive because it is a function of the estimated unknown parameter and it is also robust because it accounts for the largest possible estimation error. Of course, our raCBF is also paired with a certain parameter estimation law. 

There are a number of works on robust CBFs: \cite{xu2015rCBF, jankovic2018robust, breeden2021robust} all define a robust CBF theoretically, while ~\cite{long2022safe, hamdipoor2023safe, wei2022persistently} use SOSP to synthesize robust CBF generically for various systems. More generally, there are also other approaches to robust safety (\cite{bansal2017hamilton} uses HJB reachability to synthesize a backward reachable set under worst-case disturbances). 

There are also some works on adaptive safety. Some of these adaptive safe controllers are ad hoc and cannot guarantee safety. This is because they cannot prove that an admissible safe control input will exist at all states and for all realizations of the unknown system~\cite{xiao2021adaptive, parwana2022recursive, lyu2021merge}. By contrast, our approach ensures that there will exist a safe control input for all possible conditions, therefore guaranteeing safety. There are also theoretically-founded works on adaptive CBFs~\cite{taylor2020adaptive, maghenem2021adaptiveSafety, isaly2021multipleBF}, but these works just define different kinds of adaptive CBFs and hand-derive them for special cases. In contrast, our focus is to provide a generalizable algorithm which automatically produces raCBFs for different systems and requirements. 

% There are also various papers which use SOSP to systematically synthesize CBFs for known systems [c, c, c]. 

Our contributions are as follows:
\begin{itemize}
    \item Develop an SOS program for verifying that a given raCBF ensures safety. We extend this approach to high-degree cases and systems with multiple safety requirements.  
    \item We propose an algorithm for synthesizing raCBFs. 
    \item We validate our approach on several examples: a 2D toy system, cartpole, and 2D quadrotor. 
\end{itemize}

==> old_files/old_prob_form.tex <==
% PROBLEM FORMULATION
We use the following uncertain nonlinear system that is affine in control input and unknown model parameters \cite{lopez2023unmatched}:
\begin{equation}
    \dot x = f(x) - \Delta(x)^\top\theta + g(x)u,
\end{equation}
with state $x\in\mathbb{R}^n$, control input $u \in \mathcal{U} \subseteq \mathbb{R}^m$, known dynamics $f:\mathbb{R}^n \rightarrow \mathbb{R}^n$, unknown parameters $\theta \in \Theta \subset \mathbb{R}^p$ with known regressor $\Delta: \mathbb{R}^n \rightarrow \mathbb{R}^{p \times n}$, and known control input matrix $g: \mathbb{R}^n \rightarrow \mathbb{R}^{n\times m}$.

% The following are snippets of important backgrounds. Feel free to cut and paste and whatnot.

The following assumption is made on the unknown parameters $\theta$ \cite{lopez2023unmatched}:
\begin{assumption}
    \label{assumption:params}
    The unknown parameters $\theta$ belong to a known closed and bounded set $\Theta\subset \mathbb{R}^p$ .
\end{assumption}
Based on this assumption, we know that the parameter estimation error also belongs to a known closed and bounded set, i.e., $\Tilde{\theta} \triangleq \hat{\theta}-\theta \in \Tilde{\Theta}$. Moreover, the maximum possible parameter estimation error for each element is $\Tilde{\vartheta}_i \triangleq \underset{\Tilde{\theta}_i \in \Tilde{\Theta}}{\max} \;\Tilde{\theta}_i$ for $i=1,\dots,p$.


==> old_files/results.tex <==
\% In this section, we synthesize raCBF for three different systems: toy 2D, cartpole, and quadrotor. We show that our algorithm is quite general, producing valid raCBF for a variety of dynamics and safety specifications. We also compare closed-loop performance in simulation for our robust-adaptive controller and the baseline robust controller. We find that our robust-adaptive safety filter ensures $100\%$ safety {\it while also} interfering less with the nominal controller. This means it achieves significantly better performance on combined safety-stabilization and safety-tracking tasks. Finally, we also show that our method scales better than the baseline, handling systems of 7D as compared to 2D.      

In particular, we run two types of experiments on the closed-loop system:
\begin{enumerate}
    \item Safety test: ensure the system does not leave the invariant set under an adversarial nominal controller, which tries to drive the system out. Trials vary the initial state and the true parameter(s) value(s).
    \item Performance test: measure stabilizing/tracking performance on combined safety-(stabilizing/tracking) task. Compare with baseline, a robust CBF. Trials vary the true parameter(s) value(s).
\end{enumerate}
Results are listed in Table~\ref{} and analyzed further in the following subsections. All the experimental hyperparameters can be found in Table~\ref{} in the Appendix.

% We show that our algorithm is able to produce valid raCBF, which have large invariant sets and are robust to the desired ranges, for a variety of dynamics and safety specifications. We demonstrate in simulation that our raCBF ensures system safety, despite factors like system uncertainty and input limits. Finally, we compare our raCBF with a rCBF (robust CBF) in a feedback control experiment to illustrate that our synthesis method produces less conservative CBF.

To solve the SOSPs, we use SOSTOOLS \cite{sostools} with Mosek \cite{mosek} on a 3.00GHz Intel(R) Core(TM) i9-9980XE CPU with 16 cores and 126GB of RAM. For all examples, the initial raCBF is derived from an LQR-based CLF that stabilizes the system to the origin. Specifically, we use the solution $S$ of the algebraic Riccati equation of the system linearized about the origin to define the CLF $V(x) = x^T S x$ and the raCBF $\phi^{0}(x) = \epsilon - V(x)$, where $\epsilon \in \mathbb{R}_{>0}$ is chosen experimentally. We set the desired robust parameter ranges $\Theta$ based on the ranges of values found in the literature\cite{barto1983neuron,luuk2011quad2d}. In Fig.~\ref{fig:all_theta_across_it}, the robust range is shown to increase to the desired bounds (normalized to $0$ and $1$ for all systems). 


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/all_theta_across_it.jpg}
    \caption{Range increase of the unknown parameters across iterations for all three systems: 2D toy (green), cartpole (blue), 2D quadrotor (red). Lower bounds $\underline{\theta}$ are presented with dashed lines and upper bounds $\overline{\theta}$ are presented with solid lines. In the $y$-axis, 0 represents the desired lower-bound and 1 represents the desired upper-bound. In the $x$-axis, 0 represents the first iteration and 1 represents the last iteration.}
    \label{fig:all_theta_across_it}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Toy 2D}
We use the 2D toy system from \cite{toy2dsystem}:
\begin{equation}
    \begin{aligned}
        \dot x = \underbrace{\begin{bmatrix} x_2 - x_1^3 \\ 0 \end{bmatrix}}_{f(x)} + \underbrace{\begin{bmatrix} 0 \\ 1 \end{bmatrix}}_{g(x)} u - \underbrace{\begin{bmatrix}-x_1^2 \\ 0\end{bmatrix}}_{\Delta(x)} \theta
    \end{aligned}
\end{equation}
with $\Theta \in [0.8, 1.5]$ and $u \in [-2, 2]$. The safety definition is $\mathcal{X}_{\text{safe}} = \{ x \mid b(x) \defeq 1 - (x_1^2 + x_2^2) \ge 0 \}$.

Our synthesized raCBF attains $100\%$ safety on this system. Observe, in Fig.~\ref{fig:toy_safety_experiment}, that the trajectories under the safety-filtered adversarial controller never leave the system despite the parametric uncertainty. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Cartpole (as seen in Fig.~\ref{fig:systems_side_by_side})}\label{sec:cartpole}

For the cartpole (Fig.~\ref{fig:systems_side_by_side}), we transform the standard trigonometric dynamics~\cite{cartpole} to polynomial form by redefining the states as $[\dot x, x, {\small \dot\psi}, \sin(\psi), \cos(\psi) +1]$. For these new states, we require $\sin^2(\psi) + \cos^2(\psi) = 1$, which we incorporate into the SOSP using the S-procedure~\cite{posa2016trigsub}. The unknown parameter is the friction coefficient at the joint. We let $\Theta\in[0.28,0.31]$, following \cite{barto1983neuron} and $u\in[-5,5] N$. The safety definition confines the pole angle to be small: $\mathcal{X}_{\text{safe}} \defeq \{\sin^2(\frac{\pi}{3}) - \sin^2(\psi) \ge 0 \}$.

In Fig.~\ref{fig:cart_invariant_sets}, we plot the invariant set along $(\theta,\dot\theta)$. First, observe that the shape of the set is sensible: it is an ellipsoid with primary axis $\dot{\theta}=-\theta$, meaning it considers the pole swinging to the vertical as safe and away from the vertical as unsafe. Secondly, note that the synthesized raCBF depends meaningfully on $\hat{\theta}$. Comparing the invariant sets for $\phi(x,\ubar{\theta})$ (low joint friction) and $\phi(x,\bar{\theta})$ (high joint friction), we can see that the former set is larger. This makes sense, since for low joint friction, the pole is more responsive and easily controlled. Finally, notice that the initial invariant set is almost negligibly small, but the final set is quite large. We conclude that our algorithm is very effective at growing the invariant set.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.38\textwidth]{final_figures/cart_invariant_sets.jpg}
    \caption{The invariant sets are shown for the cartpole system: initial CBF (blue solid line), final raCBF with low joint friction coefficient (red dashed line), and final raCBF with high joint friction coefficient (red solid line).}
    \label{fig:cart_invariant_sets}
\end{figure}

As for the closed-loop simulations, raCBF attains $100\%$ safety, even with an adversarially unsafe nominal controller. We also synthesize a rCBF (robust CBF) according to \cite{kang2023verification}. In the performance test, we implement a nominal controller which controls the cart to reach position $x_{\text{goal}}$. We alternately layer the nominal controller with an raCBF-based and an rCBF-based safety filter, which both prevent the pole from tipping.

\begin{figure}[htbp]
    % \centering
    {\centering
    \includegraphics[width=0.5\textwidth]{final_figures/cart_reach_trajectories_compare_4.jpg}
    \par}
    \caption{Cartpole reach task trajectories for raCBF and rCBF. Left figure shows the cart positions of raCBF (blue) and rCBF (red). Right figure shows the pole angles of raCBF (blue) and rCBF (red). The raCBF reaches the goal states (black) faster than rCBF since it employs a larger range of pole angle.}
    \label{fig:cart_reach_trajectories_compare}
\end{figure}

\begin{figure}[htbp]
    % \centering
    {\centering
    \includegraphics[width=0.35\textwidth]{final_figures/raCBF_vs_rCBF_invariant_sets.jpg}
    \par}
    \caption{The invariant sets for raCBF (blue) and rCBF (red). Note that for a fair comparison, we used the same unknown parameter range for both controllers which is different from the one shown in Fig.~\ref{fig:cart_invariant_sets}. The invariant set of raCBF is significantly larger than that of rCBF.}
    \label{fig:raCBF_vs_rCBF_invariant_sets}
\end{figure}

Overall, the raCBF controller reaches $7.014\%$ faster. In Fig.~\ref{fig:cart_reach_trajectories_compare}, which examines one trial in detail, we see that the raCBF reaches faster because it allows a larger pole angle, which allows a larger cart acceleration. In other words, the raCBF invariant set is larger than the rCBF set (see Fig.~\ref{fig:raCBF_vs_rCBF_invariant_sets}). This is due to the difference in formulation between raCBFs and rCBFs. While both need to account for maximum estimation error, the raCBF can account for it in a more moderate way, since it utilizes parameter estimation. When the pole angle goes 

\begin{figure}[htbp]
    % \centering
    {\centering
    \includegraphics[width=0.4\textwidth]{final_figures/cart_reach_trajectory_theta_psi.jpg}
    \par}
    \caption{The parameter estimation and pole angle for raCBF in cartpole reach task. The black lines represent the upper and lower bounds of parameter, maroon line represents the true parameter value $\theta$, blue line is the estimated parameter $\hat\theta$, and the red line is the pole angle $\psi$.}
    \label{fig:cart_reach_theta_psi}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Quadrotor (as seen in Fig.~\ref{fig:systems_side_by_side})}

This system is a planar quadrotor that we transform from the typical trigonometric dynamics~\cite{luuk2011quad2d} redefining the states as $[\dot x, \dot y, \dot \psi, x, y, \sin\psi, \cos\psi - 1]$. We handle the transformation in much the same way as cartpole in Sec.~\ref{sec:cartpole}. The system has two unknown parameters, which are the drag coefficients in $x$ and $y$ and ranging in $[0, 0.01]$. The propeller thrusts are limited to $[-4, 4] mg$. The safety definition enforces the system to avoid walls on the left and right: $\mathcal{X}_{safe} = \{x \mid x < 1, x > -1\}$.

Our synthesis is able to handle a system of this moderate size (7D), producing an raCBF that ensures safety in $100\%$ of the randomized trials of the safety test (Table. ABC). The raCBF also has a large invariant set, which is evidenced by how it can track trajectories closely to the wall (Fig. WWW). On the other hand, the robust CBF from~\cite{} cannot be applied to a system of this size. However, in order to produce some point of comparison, we transfer the key parts of their formulation into our SOSP algorithm. Essentially, this just modifies the control filter feasibility constraints in phases 2 and 3 of our algorithm. This allows us to produce a result after six hours of optimization, which we use in the following performance test.

\begin{figure}[htbp]
    % \centering
    \includegraphics[width=0.5\textwidth]{final_figures/quad2d_track_raCBF_vs_rCBF.jpg}
    \caption{}
    \label{fig:quad2d_track_raCBF_vs_rCBF}
\end{figure}





















==> old_files/results_2d_poly.tex <==
% toy2dsystem

We use the 2D toy system from \cite{toy2dsystem}:
% with states $[x_1, x_2]$ and the coefficient $\theta$ as the unknown parameter, given as
\begin{equation}
    \begin{aligned}
        \dot x = \underbrace{\begin{bmatrix} x_2 - x_1^3 \\ 0 \end{bmatrix}}_{f(x)} + \underbrace{\begin{bmatrix} 0 \\ 1 \end{bmatrix}}_{g(x)} u - \underbrace{\begin{bmatrix}-x_1^2 \\ 0\end{bmatrix}}_{\Delta(x)} \theta
    \end{aligned}
\end{equation}
with $\Theta \in [0.8, 1.5]$ and $u \in [-2, 2]$. The safe definition is $\mathcal{X}_{\text{safe}} = \{ x \mid b(x) \defeq 1 - (x_1^2 + x_2^2) \ge 0 \}$. We set $\beta^{-} = -1.0$. 
% $\beta_+ = 0.5$ is used for the initial CBF. 

% We run the optimization for 11 iterations with a total computation time of 23 seconds. For each iteration, phase 1 SOS program takes approximately 0.1 second to complete, 1 second for phase 2 SOS program, and 0.8 second for phase 3 SOS program. The final raCBF is a polynomial of degree 3. 

%%% TODO: SIMIN: REWRITE %%%%%
% Fig.~\ref{fig:toy2d_levelsets} shows the invariant sets of the initial and final raCBF and trajectories from feedback control experiments using adversarial nominal controller and raCBF-QP safety-filer. As illustrated, the invariant set size noticeably increases and the difference in shape based on the unknown parameter value is evident, meaning that our raCBF is adaptive to the unknown parameter value and robust to all parameter values within the bound. All the trajectories stay within the final raCBF invariant set.
%%%%%%%%%%%%%%%%%%%%%%%%%%
% The range of the unknown parameter value for which the raCBF is robust to increases across iterations as shown in Fig.~\ref{fig:theta_across_it}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/toy2d_levelsets.jpg}
    \caption{Plot of trajectories of the feedback control experiments using adversarial nominal controller and raCBF safety-filter. The safe set and the invariant sets, represented as the zero-levelsets of the raCBF resulting from the SOS program, are shown. The safety specification (solid black line) encompasses all the invariant sets: initial CBF (dotted blue line), final raCBF with the upper parameter bound (solid red line), and final raCBF with the lower parameter bound (dashed red line). The initial state of a trajectory is shown as a dot, while the final state is shown as a X.}
    \label{fig:toy2d_levelsets}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/toy2d_theta_across_it.jpg}
%     \caption{The bound for the unknown parameter value $\theta$ increase across iterations. This shows that the raCBF synthesized from our optimization method can cover bigger unknown parameter range as iteration progresses.}
%     \label{fig:theta_across_it}
% \end{figure}

==> old_files/results_cartpole.tex <==
% Cartpole

For the cartpole (Fig.~\ref{fig:cartpole_system}), we use the dynamics from~\cite{cartpole} and transform them to be polynomial by defining our states as $[\dot x, x, {\small \dot\psi}, \sin(\psi), \cos(\psi) +1]$. After this transformation, we require that $\sin^2(\psi) + \cos^2(\psi) = 1$, which we can add to all of our SOSP constraints using the S-procedure~\cite{posa2016trigsub}. This transformation also requires us to compute the raCBF initialization using constrained LQR~\cite{scokaert1998constrained}, where the constraint is the linearization of this trigonometric identity about the origin. 

Further, we set the joint's friction coefficient as the unknown parameter. We let $\Theta \in [0.28, 0.31]$, following \cite{barto1983neuron} and $u \in [-5, 5] N$. We take $m_c = 1 kg, m_p = 0.1 kg, l=0.5m$. The safety definition constrains the pole angle: $\mathcal{X}_{\text{safe}} \defeq \{\sin^2(\frac{\pi}{3}) - \sin^2(\psi) \ge 0 \}$. We use $\beta^{-} = 0.1$.

We plot the invariant set in Fig.~\ref{fig:cartpole_levelsets} in $(\theta, \dot{\theta})$. We confirm that the shape of the set is sensible: as an ellipsoid with primary axis $\dot{\theta} = -\theta$, it considers the pole swinging back to the origin as safe and swinging away as unsafe. We also note that the raCBF depends on $\hat{\theta}$ in a sensible way - for $\hat{\theta} = \ubar{\theta}$ (smaller joint friction), the set is larger, since the pole is more responsive and easily controlled. Finally, we observe that our algorithm is very effective at growing the invariant set - whereas the initial set is almost negligibly small, the final set is quite large. 


% The invariant sets are plotted in Fig.\ref{fig:cartpole_levelsets}. We can observe that the invariant set size increases significantly after 159 iterations. For the invariant sets of the final raCBF, we see that the angular velocity increases in the opposite direction of angle so that the pole angle stays within the safe set. The difference in the invariant set sizes and shapes between the raCBF with upper parameter bound and lower parameter bound shows that the effect of the parameter value is incorporated in the final raCBF. In particular, the invariant set of $\phi_{\hat\theta}(x,\overline{\theta})$ is smaller than that of $\phi_{\hat\theta}(x,\underline{\theta})$, showing that the system is harder to keep safe when more friction is present.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/cartpole_levelsets_without_safeset}
    \caption{The invariant sets are shown for the cartpole system: initial CBF (blue solid line), final raCBF with the upper parameter bound (solid red line), and final raCBF with the lower parameter bound (dashed red line) are shown with thicker lines.} 
    % The pole angle is wrapped such that $0\le\psi\le2\pi$.}
    \label{fig:cartpole_levelsets}
\end{figure}


% The cartpole system, as shown in Fig.~\ref{fig:cartpole_system}, is based on \cite{cartpole} with the coefficient of rotational friction at the joint as the unknown parameter. The resulting rotational friction is directly proportional to the angular velocity of the pole. Thus, this model is consistent with a lubricated ball bearing joint according to \cite{cannon1967dynamics}. We define the states as $[\dot x, x, {\small \dot\psi}, \sin\psi, \cos\psi +1]$. We use trigonometric substitutions for the angle and transform coordinates such that $\Vec{0}$ is the equilibrium as shown in \cite{posa2016trigsub}.  The control input is the horizontal force on the cart along the $x$-axis and has bounds $-5\text{ N} \le u \le 5\text{ N}$. The coefficient of rotational friction is modeled to be within the set $\theta\in[0.28, 0.31]$. To account for the trigonometric substitution, an algebraic constraint $x_4^2 + (x_5-1)^2 = 1$ is added to the SOS program using the S-procedure \cite{posa2016trigsub}, \cite{dai2023convex}. We use the closed-form solution for LQR with equality constraint from \cite{posa2016constrainedLQR} to account for this algebraic constraint when constructing the CLF for the initial CBF. $\beta_+ = 0.1$ is used for the initial CBF construction. The safe set is $\mathcal{X}_{\text{safe}} = \{ x \in \mathcal{X} : \sin^2(\frac{\pi}{3}) -x_4^2 \ge 0 \}$ such that the pole angle does not deviate more than $60^\circ$ from the upright position.
% The resulting polynomial dynamics is

% \begin{equation}
%     \begin{aligned}
%         \dot x &= \underbrace{\begin{bmatrix}x_2 \\ \frac{m_p (l x_3^2 + g (x5 - 1)) x_4}{m_c + m_p x_4^2} \\ \frac{-m_p  l (x_5-1) x_3^2 x_4  - (m_c + m_p) g x_4}{(m_c + m_p x_4^2) l} \\ x_3(x_5-1) \\ -x_3 x_4\end{bmatrix}}_{f(x)} \\
%         &+ \underbrace{\begin{bmatrix}0 \\ \frac{(m_c + m_p)}{m_p l^2 (m_c + m_p x_4^2)l} \\ \frac{-(x_5 -1)}{(m_c + m_p x_4^2) l} \\ 0 \\ 0 \end{bmatrix}}_{g(x)} u - \underbrace{\begin{bmatrix}0 \\ \frac{-(x_5-1) x_2}{(m_c + m_p x_4^2)l} \\ \frac{(m_c+m_p) x_3}{m_p (m_c + m_p x_4^2)l^2} \\0 \\0 \end{bmatrix}}_{\Delta(x)^T} \theta,
%     \end{aligned}
% \end{equation}
% \begin{equation}
%     \begin{aligned}
%         \dot x &= \begin{bmatrix}\frac{m_p (l x_3^2 + g (x5 - 1)) x_4}{m_c + m_p x_4^2} \\ x_2 \\  \frac{-m_p  l (x_5-1) x_3^2 x_4  - (m_c + m_p) g x_4}{(m_c + m_p x_4^2) l} \\ x_3(x_5-1) \\ -x_3 x_4\end{bmatrix} \\
%         &+ \begin{bmatrix}\frac{1}{m_c + m_p x_4^2} \\ 0 \\ \frac{-(x_5 -1)}{(m_c + m_p x_4^2) l} \\ 0 \\ 0 \end{bmatrix} u - \begin{bmatrix}\frac{-(x_5-1) x_2}{(m_c + m_p x_4^2)l} \\ 0 \\ \frac{(m_c+m_p) x_3}{m_p (m_c + m_p x_4^2)l^2} \\0 \\0 \end{bmatrix} \theta,
%     \end{aligned}
% \end{equation}
% with system constants: mass of cart $m_c = 1$kg, mass of pole $m_p = 0.1$kg, pole length $l = 0.5$m, and gravitational acceleration $g=9.81$m/s\textsuperscript{2}. 


% Total of 159 iterations of optimization took 655 seconds to compute. For each iteration, phase 1 SOS program takes 0.12 second to complete, phase 2 SOS program takes 2.8 seconds to complete, and phase 3 SOS program takes 1.2 seconds to complete. The final raCBF is a polynomial of degree 3.
% The invariant sets are plotted in Fig.\ref{fig:cartpole_levelsets}. We can observe that the invariant set size increases significantly after 159 iterations. For the invariant sets of the final raCBF, we see that the angular velocity increases in the opposite direction of angle so that the pole angle stays within the safe set. The difference in the invariant set sizes and shapes between the raCBF with upper parameter bound and lower parameter bound shows that the effect of the parameter value is incorporated in the final raCBF. In particular, the invariant set of $\phi_{\hat\theta}(x,\overline{\theta})$ is smaller than that of $\phi_{\hat\theta}(x,\underline{\theta})$, showing that the system is harder to keep safe when more friction is present.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/cartpole_all_levelsets.jpg}
%     \caption{The invariant sets are shown for the cartpole system across the iterations (yellow lines are the initial iterations and red lines are the final iterations). The initial CBF (blue solid line), final raCBF with the upper parameter bound (solid red line), and final raCBF with the lower parameter bound (dashed red line) are shown with thicker lines.} 
%     % The pole angle is wrapped such that $0\le\psi\le2\pi$.}
%     \label{fig:cartpole_levelsets}
% \end{figure}

==> old_files/results_compare.tex <==
We compare our raCBF synthesis method with a rCBF (robust CBF) synthesis method based on \cite{kang2023verification} that is modified to fit our Alg.~\ref{alg:raCBF}. Specifically, we show that our raCBF synthesis method produces a less conservative adaptive safe controller that can improve the performance under safety-critical feedback control tasks. This is demonstrated by comparing the time-to-reach a goal location in the cartpole system while satisfying the near-upright safety specification. We conduct two sets of 200 runs for each controller, with the same initial state, goal state, and LQR nominal controller across all 400 runs. For each pair of runs (one with raCBF and the other with rCBF), the unknown friction coefficient is the same for fair comparison. On average, our raCBF reaches the goal state 8.298\% faster compared with rCBF across all runs, as illustrated in Fig.~\ref{fig:cart_compare}. This is because our raCBF is less conservative than the rCBF as illustrated by the steeper increase and decrease of velocity $\dot x$ in Fig.~\ref{fig:cart_compare}. For both experiments, the safety is preserved throughout the trajectory. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/cartpole_compare_both.jpg}
    \caption{Cartpole goal reaching task with raCBF (red solid line) and rCBF (blue dashed line) safety-filters and LQR nominal controller. The goal is to arrive 5m to the right of the origin in an upright position with zero velocity. This figure shows the runs with the median reach time from the 200 runs for each controller. Left figure illustrates the time-to-reach the goal state. Right figure shows the cart velocity with respect to the cart position.} 
    % The pole angle is wrapped such that $0\le\psi\le2\pi$.}
    \label{fig:cart_compare}
\end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}
%       \centering
%       \includegraphics[width=.5\textwidth]{figures/cartpole_comparison_t_VS_x.jpg}
%       \caption{A subfigure}
%       \label{fig:t_VS_x}
%     \end{subfigure}%
%     \begin{subfigure}
%       \centering
%       \includegraphics[width=.5\textwidth]{figures/cartpole_comparison_x_VS_xDot.jpg}
%       \caption{A subfigure}
%       \label{fig:x_VS_xDot}
%     \end{subfigure}
%     \caption{A figure with two subfigures}
%     \label{fig:cart_compare}
% \end{figure}

==> old_files/results_intro_v1.tex <==
In this section, we synthesize raCBF for three different systems: toy 2D, cartpole, and quadrotor. We show that our algorithm is able to produce valid raCBF, which have large invariant sets and are robust to the desired ranges, for a variety of dynamics and safety specifications. We demonstrate in simulation that our raCBF ensures system safety, despite factors like system uncertainty and input limits. Finally, we compare our raCBF with a rCBF (robust CBF) in a feedback control experiment to illustrate that our synthesis method produces less conservative CBF.

% We conduct raCBF synthesis and verification experiments on a 2D toy system, a cartpole, and a 2D quadrotor. 

We use SOSTOOLS \cite{sostools} with Mosek \cite{mosek} on 16 cores of Intel(R) Core(TM) i9-9980XE CPU @ 3.00GHz with 126GB of RAM to solve the SOSPs. For all examples, the initial raCBF is derived from an LQR-based CLF that stabilizes the system to the origin. Specifically, we use the solution $S$ of the algebraic Riccati equation of the system linearized about the origin to define the CLF $V(x) = x^T S x$ and the raCBF $\phi^{0}(x) = \epsilon - V(x)$, where $\epsilon \in \mathbb{R}_{>0}$ is chosen experimentally. We set the desired robust parameter ranges $\Theta$ using commonly known ranges for the physical parameter values \cite{barto1983neuron,luuk2011quad2d}. In Fig.~\ref{fig:all_theta_across_it}, the robust range is shown to increase to the desired bounds (normalized to $0$ and $1$ for all systems). 
% The range $\Theta$ of the unknown parameters increase to the full admissible range at the end of optimization as shown in Fig.~\ref{fig:all_theta_across_it}.  

% for the linearized system about the origin to construct the CLF such that $V(x) = x^T S x$. Then the initial CBF is constructed as $\phi_{\hat\theta}(x) = \beta_+ - V(x)$, where $\beta_+ \in \mathbb{R}_{>0}$. The range $\Theta$ of the unknown parameters increase to the full admissible range at the end of optimization as shown in Fig.~\ref{fig:all_theta_across_it}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/all_theta_across_it.jpg}
    \caption{Range increase of the unknown parameters across iterations for all three systems: 2D toy (green), cartpole (blue), 2D quadrotor (red). Lower bounds $\underline{\theta}$ are presented with dashed lines and upper bounds $\overline{\theta}$ are presented with solid lines. In the $y$-axis, 0 represents the desired lower-bound and 1 represents the desired upper-bound. In the $x$-axis, 0 represents the first iteration and 1 represents the last iteration.}
    \label{fig:all_theta_across_it}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}
%         \includegraphics[width=0.25\textwidth]{figures/toy2d_theta_across_it.jpg}
%     \end{subfigure}
    
%     \begin{subfigure}
%         \includegraphics[width=0.25\textwidth]{figures/cartpole_theta_across_it.jpg}
%     \end{subfigure}
    
%     \begin{subfigure}
%         \includegraphics[width=0.25\textwidth]{figures/quad2d_theta_across_it.jpg}
%     \end{subfigure}
    
%     \caption{The bound for the unknown parameter value $\theta$ increase across iterations. This shows that the raCBF synthesized from our optimization method can cover bigger unknown parameter range as iteration progresses.}
%     \label{fig:theta_across_it}
% \end{figure}

==> old_files/results_intro_v2.tex <==
In this section, we synthesize raCBF for three different systems: toy 2D, cartpole, and quadrotor. We show that our algorithm is quite general, producing valid raCBF for a variety of dynamics and safety specifications. We also compare closed-loop performance in simulation for our robust-adaptive controller and the baseline robust controller. We find that our robust-adaptive safety filter ensures $100\%$ safety {\it while also} interfering less with the nominal controller. This means it achieves significantly better performance on combined safety-stabilization and safety-tracking tasks. Finally, we also show that our method scales better than the baseline, handling systems of 7D as compared to 2D.      

In particular, we run two types of experiments on the closed-loop system:
\begin{enumerate}
    \item 
    \item 
\end{enumerate}


% We show that our algorithm is able to produce valid raCBF, which have large invariant sets and are robust to the desired ranges, for a variety of dynamics and safety specifications. We demonstrate in simulation that our raCBF ensures system safety, despite factors like system uncertainty and input limits. Finally, we compare our raCBF with a rCBF (robust CBF) in a feedback control experiment to illustrate that our synthesis method produces less conservative CBF.

We use SOSTOOLS \cite{sostools} with Mosek \cite{mosek} on 16 cores of Intel(R) Core(TM) i9-9980XE CPU @ 3.00GHz with 126GB of RAM to solve the SOSPs. For all examples, the initial raCBF is derived from an LQR-based CLF that stabilizes the system to the origin. Specifically, we use the solution $S$ of the algebraic Riccati equation of the system linearized about the origin to define the CLF $V(x) = x^T S x$ and the raCBF $\phi^{0}(x) = \epsilon - V(x)$, where $\epsilon \in \mathbb{R}_{>0}$ is chosen experimentally. We set the desired robust parameter ranges $\Theta$ using commonly known ranges for the physical parameter values \cite{barto1983neuron,luuk2011quad2d}. In Fig.~\ref{fig:all_theta_across_it}, the robust range is shown to increase to the desired bounds (normalized to $0$ and $1$ for all systems). 


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/all_theta_across_it.jpg}
    \caption{Range increase of the unknown parameters across iterations for all three systems: 2D toy (green), cartpole (blue), 2D quadrotor (red). Lower bounds $\underline{\theta}$ are presented with dashed lines and upper bounds $\overline{\theta}$ are presented with solid lines. In the $y$-axis, 0 represents the desired lower-bound and 1 represents the desired upper-bound. In the $x$-axis, 0 represents the first iteration and 1 represents the last iteration.}
    \label{fig:all_theta_across_it}
\end{figure}

==> old_files/results_quad2d.tex <==
% quadrotor 2D
The final experiment is with a planar quadrotor with 7 states $[\dot x, \dot y, \dot \psi, x, y, \sin\psi, \cos\psi - 1]$ based on \cite{drake}, with the drag coefficients along the $x$ and $y$ directions as the unknown parameters as shown in \cite{luuk2011quad2d}. The thrust forces of the two propellers are the control inputs with bounds $-4 \;mg \le u_i \le 4 \; mg, \;i=1,2$. Trigonometric substitution is used for the angle and change-of-coordinates is performed to account for the gravitational acceleration in the $y$-direction so that the equilibrium is $\Vec{0}$ with stead-state input $\Vec{0}$. The drag coefficients are within the set $\theta_i \in [0, 0.01],\; i=1,2$. The algebraic constraint $x_6^2 + (x_7 + 1)^2 = 1$ is added to the SOS program to account for the trigonometric substitution, as explained in the previous cartpole example. The closed-form solution for LQR with equality constraint is used to construct the CLF for the initial CBF with $\beta_+ = 0.05$. We design two safety specifications such that the center of the quadrotor avoids hitting two vertical walls, each 1 m away from the origin. Thus, the safe set is defined as $\mathcal{X}_{\text{safe}} = \{ x\in\mathcal{X} : x_4 + 1 \ge 0, 1 - x_4 \ge 0 \}$. 
% The resulting polynomial dynamics for the 2D quadrotor is
% {\small
% \begin{equation}
%     \begin{aligned}
%         \dot x = \begin{bmatrix} -x_6 g \\ (x_7+1) g \\ 0 \\ x_1 \\ x_2 \\ (x_7+1) x_3 \\ -x_6 x_3 \end{bmatrix}
%         + \begin{bmatrix} \frac{-x_6}{m} & \frac{-x_6}{m} \\ \frac{x_7+1}{m} & \frac{x_7+1}{m} \\ \frac{r}{I} & \frac{-r}{I} \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \end{bmatrix} \begin{bmatrix} u_1 \\ u_2 \end{bmatrix} - \begin{bmatrix} x_1 & 0 \\ 0 & x_2 \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \\ 0 & 0 \end{bmatrix} \begin{bmatrix} \theta_1 \\ \theta_2 \end{bmatrix},
%     \end{aligned}
% \end{equation}
% }
% with mass $m = 0.486$kg, length of the rotor arm $r = 0.25$m, moment of inertia $I = 0.00383$kg$\cdot$m\textsuperscript{2}, and gravitational acceleration $g=9.81$m/s\textsuperscript{2}. 

% Synthesizing a raCBF took 337 iterations for 68,934 seconds, with 0.87 seconds of computation for phase 1 SOS program, 74 seconds for phase 2 SOS program, and 130 seconds for phase 3 SOS program in each iteration. 
Due to the computational limitations of the software packages, we `trimmed' the lagrange multipliers and $\phi_{\hat{\theta}}$ in each phase by dropping terms with coefficients smaller than 0.001. The final raCBF is used for a reference-tracking experiment with LQR as the nominal controller, as illustrated in Fig.\ref{fig:quad2d_trajectory}. The reference is a circle with radius 2.5m about the origin. The raCBF-QP safety filter ensures that the center of the quadrotor never collides with either wall while following the trajectory. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/quad2d_trajectory.jpg}
    \caption{Trajectory of the 2D quadrotor (solid blue line) is shown for trajectory-tracking with LQR as the nominal controller and raCBF-QP as the safety filter. The reference trajectory (dashed red line) is a circle about the origin with radius 2.5m. The angle of the quadrotor is measured with respect to the positive $x$-axis and is positive in counter-clockwise direction.}
    \label{fig:quad2d_trajectory}
\end{figure}

==> old_files/results_table.tex <==

%%%% NOTE: apparently this table caption format is the official formatting of IEEEconf. It's actually supposed to be all small caps, but I changed it. %%%%



%%%%%%%%%%%%%%% Adversarial Safety Metric %%%%%%%%%%%%%%%
\begin{table}[!ht]
\centering
    \caption{}
    \label{tab:fb_metric}
    \begin{tabular}{|c||c|c|c|}
         \hline
           &  Results for Feedback Simulations  \\
         \hhline{|=||=|=|=|}
         \begin{tabular}{@{}c@{}} Safety \% \\ (Number of runs) \end{tabular} & \begin{tabular}{@{}c@{}}100\% \\ (200) \end{tabular} & \begin{tabular}{@{}c@{}}100\% \\ (200) \end{tabular} & \begin{tabular}{@{}c@{}}100\% \\ (200) \end{tabular} \\
         \hline
    \end{tabular}
\end{table}

%%%%%%%%%%%%%%% Performance Safety Metric %%%%%%%%%%%%%%%
\begin{table}[!ht]
\centering
    \caption{Performance comparison between raCBF and rCBF for cartpole reach task and 2D quadrotor tracking task. NEED BETTER NAMING FOR COLUMNS AND ROWS.}
    \label{tab:safety_metric}
    \begin{tabular}{|c||c|c|}
         % \hline
         %  Results & \begin{tabular}{@{}c@{}}raCBF\\(Avg.) \end{tabular} & \begin{tabular}{@{}c@{}}rCBF\\(Avg.) \end{tabular}  & \begin{tabular}{@{}c@{}} Upper\\Bound (Avg.) \end{tabular}  & \begin{tabular}{@{}c@{}} raCBF vs rCBF \\ (Avg.\%) \end{tabular}\\
          
         % \hhline{|=||=|=|=|=|}
         
         % \begin{tabular}{@{}c@{}} Cartpole\\Reach Time \end{tabular} & 14.87 s & 13.83 s & 13.64 s & 7.01387\%\\ 
         
         % \hline
         
         % \begin{tabular}{@{}c@{}} Quadrotor\\Track Error \end{tabular} \\
         
         % \hline

         \hline
          Results & Cartpole Reach Time & Quadrotor Track Error\\
         \hhline{|=||=|=|}
         \begin{tabular}{@{}c@{}}raCBF\\(Avg.) \end{tabular} & 13.82671 sec & \\ 
         \hline
         \begin{tabular}{@{}c@{}}rCBF\\(Avg.) \end{tabular} & 
         14.86958 sec & \\
         \hline
         \begin{tabular}{@{}c@{}} Upper Bound \\ (Avg.) \end{tabular} & 13.64022 sec & \\
         \hline
         \begin{tabular}{@{}c@{}} raCBF vs rCBF \\ (Avg. Rate) \end{tabular} & 7.01387\% & \\
         \hline
         \begin{tabular}{@{}c@{}} raCBF vs rCBF \\ (Avg. Var) \end{tabular} & 0.04002\% & \\
         \hline
    \end{tabular}
\end{table}


==> old_files/v0_intro.tex <==
% INTRODUCTION

There is a noticeable lack of practical safe control methods for uncertain systems. While much theory has been developed on this problem, these theoretical works do not actually give a generalizable means for \textit{producing} safe controller \cite{lopez2023unmatched, ames2020aCBF}. This is problematic, since we desire safety for many robotic systems that have unmeasurable system parameters. For example, robotic arms and autonomous vehicles have to avoid collisions with humans, but their dynamical models have unknown frictional coefficients \cite{}. Our work fills this fundamental gap. We leverage sums-of-squares programming to synthesize safe controllers for any parameter-affine uncertain system. 

Theoretical works for addressing system uncertainty generally fall into one of three categories: adaptive safety \cite{maghenem2021adaptiveSafety, isaly2021multipleBF, black2021adaptLaw}, robust safety \cite{xu2015rCBF, jankovic2018robust, breeden2021robust}, or a combination of the two \cite{lopez2020RaCBF, cohen2022HoRaCBF}. Generally, these works solely focus on deriving conditions that an adaptive or robust CBF must satisfy. They do not cover the separate `synthesis problem,' which is about designing algorithms to generate CBFs to satisfy these theoretical conditions. These synthesis algorithms are highly generic tools: given any system satisfying some assumptions, they can produce a valid CBF. In contrast, these theoretical works only derive CBFs for very special (small and simple) cases.

For synthesis, we use sum-of-squares programming (SOSP), which is a special kind of optimization. Given the CBF as a parametrized function, SOSP can optimize for valid parameters.       

% I don't particularly see any paper on SOSP rCBF, except the Harvard Paper
Uncertain systems have long been handled with either adaptive or robust control (or a combination of the two) \cite{astrom2008adaptive, lavretsky2012robustAdaptive}. These paradigms are quite different. In the adaptive scheme, the controller depends on the current estimated system. (Hence, adaptive control also studies parameter estimation.) On the other hand, in robust control, the controller depends only on some assumed “worst-case” system. While there are a few works on robust safety synthesis (\cite{} uses SOSP to synthesize a robust CBF, and \cite{choi2021rCBVF} uses HJB reachability to synthesize a robust backward reachable set), there are no corresponding works on adaptive safety synthesis, to our knowledge. Adaptive CBF is currently limited to theory and hence, quite impractical. This is a significant shortcoming of the literature, since there are many scenarios where adaptive control is more suitable than robust control. 
% Page 426, Ch. 10 of the textbook.
For example, adaptive control excels when the range of the unknown dynamics is large \cite{astrom2008adaptive}.

There are also a number of adaptive safety works that lack guarantees \cite{xiao2021adaptive, lyu2021merge}. These are generally “self-tuning” approaches, where the controller and estimator are designed separately (choose some controller, some estimator). A self-tuning controller typically only ensures safety under the estimated dynamics, not the actual dynamics. In order to attain safety under the actual dynamics, we would have to reason about the difference between estimated and actual dynamics. Some works attempt to do just that: for example, \cite{} [c: Changliu DSCC, Qin recent] estimate a set that the true dynamics is likely to lie in (robust adaptive control). However, none of these methods can ensure that the actual dynamics is captured within the estimates and therefore cannot have safety guarantees. In contrast, the approach we use jointly designs the controller and estimator, which facilitates the safety proof \cite{lopez2023unmatched}. Using this joint design, we actually do not have to reason about the accuracy of the estimator. 

Another common issue with existing adaptive safety methods is that for certain estimated/actual dynamics, a safe control input may not exist within the physical actuation limits [c, c, c]. We address this potential issue as well. Our algorithm ensures that there will always exist a safe control input, no matter the value of the current estimated dynamics.  

